Self-balanced Learning For Domain Generalization

Domain generalization aims to learn a prediction model on multi-domain source data such that the model can generalize to a target domain with unknown statistics. Most existing approaches have been developed under the assumption that the source data is well-balanced in terms of both domain and class. However, real-world training data collected with different composition biases often exhibits severe distribution gaps for domain and class, leading to substantial performance degradation. In this paper, we propose a self-balanced domain generalization framework that adaptively learns the weights of losses to alleviate the bias caused by different distributions of the multi-domain source data. The self-balanced scheme is based on an auxiliary reweighting network that iteratively updates the weight of loss conditioned on the domain and class information by leveraging balanced meta data. Experimental results demonstrate the effectiveness of our method overwhelming state-of-the-art works for domain generalization.

==> table.tex <==



\begin{table}[t]
    \caption{The classification accuracy on VLCS dataset.}
    \centering
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{lccccc}
        \hlinewd{0.8pt}
        \textbf{Method}   & \textbf{C}           & \textbf{L}           & \textbf{S}           & \textbf{V}           & \textbf{Avg}         \\
        \hline \hline
        CIDDG\cite{li2017deeper}                 & 88.83       & 63.06       & 62.10       & 64.38       & 69.59                 \\
        Undo-Bias\cite{li2017deeper}                 & 93.63       & 63.49       & 61.32       & 69.99       & 72.11                 \\
        MMD-AAE\cite{mmd-aae}                 & 94.40       & 62.60       & 64.40       & 67.70       & 72.28                 \\
        MLDG\cite{mldg}                 & 94.40       & 61.30       & 65.90       & 67.70       & 72.30                 \\
        Epi-FCR\cite{epifcr}                 & 94.10       & 64.30       & 65.90       & 67.10       & 72.90                 \\
        JiGen\cite{jigsaw}                 & 96.93       & 60.90       & 64.30       & 70.62       & 73.19                 \\
        MASF\cite{masf}                 & 94.78       & 64.90       & 67.64       & 69.14       & 74.11                 \\
        RSC\cite{RSC}            & 97.61       & 61.86       & 68.32       & \textbf{73.93}       & 75.43                 \\ \hline
        Ours(RSC)            & \textbf{97.92}       & \textbf{65.22}       & \textbf{70.98}       & 70.18       & \textbf{76.08}                 \\
        \hlinewd{0.8pt}
        \end{tabular}
    }
    \label{tab:vlcs}
    \vspace{-7pt}
\end{table}


\begin{table}[t]
    \caption{Abalation study for the effect of conditional domain vector on VLCS dataset. Baseline method is RSC~\cite{}.}
    \centering
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{ccccccc}
        \toprule
        \textbf{Domain vector}   & \textbf{C}           & \textbf{L}           & \textbf{S}           & \textbf{V}           & \textbf{Avg}         \\
        \midrule
        \xmark             & \textbf{97.88 $\pm$ 0.1}       & 61.32 $\pm$ 0.9       & 68.12 $\pm$ 0.9       & 70.86 $\pm$ 2.5       & 74.545                 \\
        \cmark            & 97.62 $\pm$ 0.3       & \textbf{64.92 $\pm$ 0.3}       & \textbf{68.98 $\pm$ 0.1}       & \textbf{70.88 $\pm$ 0.3}       & \textbf{75.60}                 \\
        \bottomrule
        \end{tabular}
    }
    \label{tab:tab2}
\end{table}






% \begin{table}[t]
%     \centering
%     \resizebox{1\linewidth}{!}{
%         \begin{tabular}{lcccccc}
%         \toprule
%         \textbf{Domain vector}   & \textbf{C}           & \textbf{L}           & \textbf{S}           & \textbf{V}           & \textbf{Avg}         \\
%         \midrule
%         MLDG                 & 97.9 $\pm$ 0.3       & 60.3 $\pm$ 1.3       & 68.6 $\pm$ 1.5       & 72.4 $\pm$ 0.6       & 74.8                 \\
%         \xmark             & 97.7 $\pm$ 0.1       & 61.9 $\pm$ 0.9       & 68.6 $\pm$ 0.9       & 71.4 $\pm$ 2.5       & 74.9                 \\
%         \cmark            & 97.6 $\pm$ 0.3       & 65.2 $\pm$ 0.3       & 70.2 $\pm$ 0.1       & 70.8 $\pm$ 0.3       & 75.95                 \\
%         RSC+SBDG            & 94.56 $\pm$ 0.4       & 64.87 $\pm$ 0.3       & 68.29 $\pm$ 0.1       & 69.04 $\pm$ 0.1       & 74.19                 \\
%         \bottomrule
%         \end{tabular}
%     }
%     \caption{Abalation study for the effect of components in our method on VLCS dataset. MLDG is a reproduced score of our experiment. Model selection methods : Training-domain best validation score}
    
%     \label{tab:vlcs2}
    
% \end{table}









% \subsubsection{PACS}

% \begin{center}
% \adjustbox{max width=\linewidth}{%
% \begin{tabular}{lccccc}
% \toprule
% \textbf{Method}   & \textbf{A}           & \textbf{C}           & \textbf{P}           & \textbf{S}           & \textbf{Avg}         \\
% \midrule
% MMD-AAE                 & 75.2       & 72.7       & 96       & 64.2       & 77                 \\
% CCSA                 & 80.5       & 76.9       & 93.6       & 66.8       & 79.5                 \\
% JiGen                 & 79.42       & 75.25       & 96.03       & 71.35       & 80.51                 \\
% CrossGrad                 & 79.8       & 76.8       & 96       & 70.2       & 80.7                 \\
% D-SAM                 & 77.33       & 72.43       & 95.3       & 77.83       & 80.72                 \\
% MASF                 & 80.29       & 77.17       & 94.99       & 71.69       & 81.03                 \\
% DMG                 & 76.9       & 80.38       & 93.35       & 75.21       & 81.46                 \\
% Epi-FCR                 & 82.1       & 77       & 93.9       & 73       & 81.5                 \\
% MetaReg                 & 83.7       & 77.2       & 95.5       & 70.3       & 81.7                 \\
% MMLD                 & 81.28       & 77.16       & 96.09       & 72.29       & 81.83                 \\
% EISNet                 & 81.89       & 76.44       & 95.93       & 74.33       & 82.15                 \\
% L2A-OT                 & 83.3       & 78.2       & 96.2       & 73.6       & 82.8                 \\
% DDAIG                 & 84.2       & 78.1       & 95.3       & 74.7       & 83.1                 \\
% RSC                 & 83.43       & 80.31       & 95.99       & 80.85       & 85.15                 \\
% MLDG_{reproduce}                 & 79.7 $\pm$ 0.2       & 70.3 $\pm$ 1.0       & 94.2 $\pm$ 0.1       & 71.9 $\pm$ 0.5       & 79.03                 \\
% MWN+MLDG             & 78.9 $\pm$ 0.8       & 71.2 $\pm$ 0.4       & 94.7 $\pm$ 0.4       & 68.9 $\pm$ 0.1       & 78.43                 \\
% CMWN+MLDG            & 80.2 $\pm$ 0.8       & 71.5 $\pm$ 0.3       & 95.5 $\pm$ 0.1       & 71.9 $\pm$ 0.1       & 79.78                 \\
% CMWN+RSC*(batch48)            & 76.56       & 77.94       & 93.29       & 82.97       & 82.69                 \\
% CMWN+RSC**(batch48)            & 80.47       & 80.67       & 94.13       & 83.23       & 84.63                 \\
% CMWN+RSC*(batch64)            & 78.61       & 78.8       & 94.37       & 74.65       & 81.61                 \\
% CMWN+RSC**(batch64)            & 82.37       & 78.97       & 94.73       & 81.24       & 84.33                 \\
% \bottomrule
% \end{tabular}}
% \caption{DG results on PACS dataset(Resnet-18), Model selection methods : Training-domain best validation score}
% \end{center}

% \subsubsection{Averages}

% \begin{center}
% \adjustbox{max width=\textwidth}{%
% \begin{tabular}{lccc}
% \toprule
% \textbf{Algorithm}        & \textbf{VLCS}             & \textbf{PACS}             & \textbf{Avg}              \\
% \midrule
% MLDG                      & 72.3            & 80.7            & 76.5                      \\
% MWNMLDG                      & 74.9 $\pm$ 0.6            & 78.4 $\pm$ 0.2            & 76.65                      \\
% \bottomrule
% \end{tabular}}
% \end{center}

